Temporal Variational Implicit Neural Representations

We introduce Temporal Variational Implicit Neural Representations (TV-INRs), a probabilistic framework for modeling irregular multivariate time series that enables efficient and accurate individualized imputation and forecasting. By integrating implicit neural representations with latent variable models, TV-INRs learn distributions over time-continuous generator functions conditioned on signal-specific covariates. Unlike existing INR approaches that require extensive training, fine-tuning or meta-learning, our method achieves accurate individualized predictions through a single forward pass. Our experiments demonstrate that with a single TV-INRs instance, we can accurately solve diverse imputation and forecasting tasks, offering a computationally efficient and scalable solution for real-world applications. TV-INRs performs particularly well in low-data regimes, where on several datasets it achieves substantially lower imputation error, including order-of-magnitude improvements.

==> annotate-equations.tex <==
% Annotate LaTeX Equations
% 
% (c) 2022 by ST John, https://github.com/st--/
% Licensed under MIT License
% 
\NeedsTeXFormat{LaTeX2e}[1994/06/01]
\ProvidesPackage{annotate-equations}
  [2023/05/06 v0.2.2 easily annotate equations using TikZ]

%%% lualatex compatibility, from https://tex.stackexchange.com/a/351520/171664
\RequirePackage{ifluatex}
\ifluatex
\RequirePackage{luatex85}
\RequirePackage{pdftexcmds}
  \makeatletter
  \let\pdfstrcmp\pdf@strcmp
  \let\pdffilemoddate\pdf@filemoddate
  \makeatother
\fi
%%%

\RequirePackage{tikz}
\RequirePackage{xcolor}

\usetikzlibrary{backgrounds}
\usetikzlibrary{arrows,shapes}
\usetikzlibrary{tikzmark} % for \tikzmarknode
\usetikzlibrary{calc} % for computing the midpoint between two nodes, e.g. at ($(p1.north)!0.5!(p2.north)$) 


%%%%% SETTINGS %%%%%

\newcommand{\eqnhighlightheight}{}  % colorbox will shrink to content
\renewcommand{\eqnhighlightheight}{\mathstrut} % colorbox will always have full height

\newcommand{\eqnhighlightshade}{17}  % light
%\renewcommand{\eqnhighlightshade}{47}  % dark

\newcommand{\eqnannotationstrut}{\strut} % Package default
\newcommand{\eqnannotationfont}{\sffamily\footnotesize}


\providecommand\EAmarkanchor{north} % default set to "above"
\providecommand\EAwesteast{east} % default set to "right"
\providecommand\EAlabelanchor{south} % default set to "label above"
% for pgfkeys, see https://tex.stackexchange.com/a/34318/171664
% for no-value keys, see https://tex.stackexchange.com/a/401848/171664
\pgfkeys{
    /eqnannotate/.is family, /eqnannotate,
    above/.code = {\renewcommand\EAmarkanchor{north}},
    below/.code = {\renewcommand\EAmarkanchor{south}},
    left/.code = {\renewcommand\EAwesteast{west}},
    right/.code = {\renewcommand\EAwesteast{east}},
    label above/.code = {\renewcommand\EAlabelanchor{south}},
    label below/.code = {\renewcommand\EAlabelanchor{north}},
}

\tikzset{annotate equations/arrow/.style={}}
\tikzset{annotate equations/text/.style={font=\eqnannotationfont}}

%%%%% %%%%%%%% %%%%%


\newcommand*{\eqnhighlightcolorbox}[2]{%
% \colorbox sets the second argument in text mode, so for use within equations we wrap it in $ $ again
    \mathchoice% to get right font size in each mode:
        {\colorbox{#1}{$\displaystyle #2$}}%
        {\colorbox{#1}{$\textstyle #2$}}%
        {\colorbox{#1}{$\scriptstyle #2$}}%
        {\colorbox{#1}{$\scriptscriptstyle #2$}}%
}

%%% the fbox with 0pt rule fixes the height of eqnmark vs eqnmarkbox issue
\newcommand*{\eqnhighlightfbox}[2]{%
% \fbox sets the second argument in text mode, so for use within equations we wrap it in $ $ again
    \mathchoice% to get right font size in each mode:
        {\begingroup\setlength{\fboxrule}{0pt}\fbox{$\displaystyle\color{#1}#2$}\endgroup}%
        {\begingroup\setlength{\fboxrule}{0pt}\fbox{$\textstyle\color{#1}#2$}\endgroup}%
        {\begingroup\setlength{\fboxrule}{0pt}\fbox{$\scriptstyle\color{#1}#2$}\endgroup}%
        {\begingroup\setlength{\fboxrule}{0pt}\fbox{$\scriptscriptstyle\color{#1}#2$}\endgroup}%
}

% . is the current color

\newcommand*{\eqnhighlight}[2]{\begingroup\colorlet{currentcolor}{.}\eqnhighlightcolorbox{#1!\eqnhighlightshade}{\eqnhighlightheight #2}\endgroup}
\newcommand*{\eqncolor}[2]{\begingroup\colorlet{currentcolor}{.}\eqnhighlightfbox{#1}{\eqnhighlightheight #2}\endgroup}

%%% Arguments to \eqnmark[box]: [highlight color]{node name}{term to highlight}
\newcommand*{\eqnmarkbox}[3][currentcolor]{\addvalue{#2}{#1}\tikzmarknode{#2}{\eqnhighlight{#1}{#3}}}
\newcommand*{\eqnmark}[3][currentcolor]{\addvalue{#2}{#1}\tikzmarknode{#2}{\eqncolor{#1}{#3}}}

% Store current color in a dictionary (lookup table),
% from https://tex.stackexchange.com/a/48931/171664 :
\def\addvalue#1#2{\expandafter\gdef\csname eqnannotate@data@#1\endcsname{#2}}
\def\usevalue#1{%
  \ifcsname eqnannotate@data@#1\endcsname
    \csname eqnannotate@data@#1\expandafter\endcsname
  \else
    currentcolor%
  \fi
}


%%%%% Helpers for swapping north/south / west/east / -/+ depending on above/below / left/right etc.:
\newcommand*{\swapNorthSouth}[1]{%
    \ifnum\pdfstrcmp{#1}{south}=0 north\else south\fi
}
\newcommand*{\swapWestEast}[1]{%
    \ifnum\pdfstrcmp{#1}{east}=0 west\else east\fi
}
\newcommand*{\EAxshift}[1]{%
    \ifnum\pdfstrcmp{#1}{east}=0 -0.3ex\else 0.3ex\fi
}
%%%%%


\newcounter{eqnannotatenode}
\newcommand*{\eqnannotateCurrentNode}{eqnannotatenode\theeqnannotatenode}


\newcommand{\annotatetwo}[5][]{%
    \begingroup% %%% so we don't leak the \def's below
    \stepcounter{eqnannotatenode}%
    %%% #1: (optional) extra args for \node e.g. yshift=...
    \pgfkeys{/eqnannotate, #2}% %%% all configuration options
    \def\myEAmarkOne{#3}%
    \def\myEAmarkTwo{#4}%
    \colorlet{currentcolor}{.}
    \def\myEAtext{#5}%
    \def\myEAcolor{\usevalue{\myEAmarkOne}}%
    \begin{tikzpicture}[overlay,remember picture,>=stealth,nodes={align=left,inner ysep=1pt},<-]
        % default anchor is at center
		\node[anchor=\swapNorthSouth{\EAmarkanchor},color=\myEAcolor!85,
			annotate equations/text,#1
			]  % color blended with white to 85%, any (optional) extra args #1
            (\eqnannotateCurrentNode)   % use counter-based "local node"
            at ($(\myEAmarkOne.\EAmarkanchor)!0.5!(\myEAmarkTwo.\EAmarkanchor)$)  % centered between the two nodes
            {\myEAtext\eqnannotationstrut};
        % double arrow to two uses within the equation:
        \draw [<->,color=\myEAcolor, annotate equations/arrow] (\myEAmarkOne.\EAmarkanchor) |- ([yshift=0.1ex] \eqnannotateCurrentNode.\EAlabelanchor) -| (\myEAmarkTwo.\EAmarkanchor);  % from node 1 via annotation to node 2, with anchor #6 each
    \end{tikzpicture}%
    \endgroup% %%% close group again
}


%%% \extractfirst from https://tex.stackexchange.com/a/115733/171664
\RequirePackage{expl3}
\RequirePackage{xparse}
\ExplSyntaxOn
\NewDocumentCommand{\extractfirst}{mm}
 {
  \tl_set:Nx #1 {\clist_item:Nn #2 { 1 } }
 }
\ExplSyntaxOff
%%%

\newcommand{\annotate}[4][]{%
    \begingroup% %%% so we don't leak the \def's below
    \stepcounter{eqnannotatenode}%
    %
    %
    %
    % #1: (optional) extra args for \node e.g. yshift=...
    \pgfkeys{/eqnannotate, #2}%
    \def\myEAmarks{#3}%
    \extractfirst\myEAmark\myEAmarks% %%% get first node for color and annotation
    \def\myEAtext{#4}%
    %
    %
    \colorlet{currentcolor}{.}%
    \def\myEAcolor{\usevalue{\myEAmark}}%
    %
    \def\EAspace{ }% workaround: did not find any other way of getting a space into \myEAlabelanchor without upsetting LaTeX/PGF/... somehow
    \edef\myEAlabelanchor{\EAlabelanchor\EAspace\EAwesteast}%
    %
    %
    \def\myEAxshift{\EAxshift{\EAwesteast}}%
    \begin{tikzpicture}[overlay,remember picture,>=stealth,nodes={align=left,inner ysep=1pt},<-]
		\node[anchor=\swapNorthSouth{\EAmarkanchor} \swapWestEast{\EAwesteast},
			color=\myEAcolor!85,annotate equations/text,#1] % TODO for some reason, passing #1 through command doesn't work...
                % anchor=west: align left edge of text on top of tikzmark in equation
                % should be north west for below and south west for above ...
            (\eqnannotateCurrentNode) at (\myEAmark.\EAmarkanchor)  % \EAmarkanchor north: above the equation, south: below
            {\myEAtext\eqnannotationstrut};
        \foreach \EAmark in \myEAmarks
        \draw [color=\myEAcolor, annotate equations/arrow] (\EAmark.\EAmarkanchor)  % arrow from the equation
                % \EAmarkanchor north: above the equation, south: below
            |- ([xshift=\myEAxshift,yshift=0.1ex] \eqnannotateCurrentNode.\myEAlabelanchor);
                % - south east: we want line to end at bottom right of annotation text;
                % - negative xshift makes it a little bit shorter;
                % - yshift for aesthetics (\strut is ever so slightly too tall).
    \end{tikzpicture}%
    \endgroup% %%% close group again
}

\endinput
%%
%% End of file


==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> my_commands.tex <==
\usepackage{tabularx}       % Tables
\usepackage{booktabs} 

\newcommand{\ours}{TV-INRs{}}
\newcommand{\oursc}{C-TV-INRs{}}
\newcommand{\oursfull}{Temporal Variational Implicit Neural Representations{}}
\newcommand{\oursfulllower}{Temporal variational implicit neural representations}


% Define colors for different authors
\definecolor{color_batu}{RGB}{0,0,128} % Red
\definecolor{color_rachael}{RGB}{0,128,0} % Green
\definecolor{color_all}{RGB}{255,255,50} % Green
% Define more colors if needed

\newcommand{\rdv}[1]{\textcolor{color_rachael}{\textbf{RV:} #1}}

\newenvironment{rebuttal}%
  {\color{black}\ignorespaces}%
    % {\color{orange}\ignorespaces}%
  {\unskip}


\newenvironment{tmlr}%
  {\color{black}\ignorespaces}%
    % {\color{orange}\ignorespaces}%
  {\unskip}

\newenvironment{tmlr2}%
  {\color{black}\ignorespaces}%
    % {\color{purple}\ignorespaces}%
  {\unskip}

\newenvironment{tmlr3}%
  {\color{black}\ignorespaces}%
    % {\color{green}\ignorespaces}%
  {\unskip}
  
%adding citations:
\newcommand{\addcitation}[1]{\textcolor{blue}{[Add Citation: #1]}}
% \newcommand{\ourmodel}{\textsc{MuStP}}
% \newcommand{\labdata}{\textsc{LabData}}
% \newcommand{\everydaydata}{\textsc{EverydayData}}
% \newcommand{\devicewatch}{\textsc{Withings ScanWatch}}
% \newcommand{\devicelab}{\textsc{Zephyr Bioharness 3.0}}
% \newcommand{\neurokittwo}{\textsc{NeuroKit2}}


%%%%%%%%%%  MATHCAL
\newcommand{\Lcal}{\mathcal{L}}
\newcommand{\Xcal}{\mathcal{X}}
\newcommand{\Ycal}{\mathcal{Y}}
\newcommand{\Tcal}{\mathcal{T}}

%%%%%%%%%% BOLD SPECIAL CHARACTERS
\newcommand{\thetab}{\boldsymbol{\theta}}
\newcommand{\phib}{\boldsymbol{\phi}}
\newcommand{\etab}{\boldsymbol{\eta}}

\newcommand{\gammab}{\boldsymbol{\gamma}}
\newcommand{\gammabz}{\gammab_{z}}
\newcommand{\gammabc}{\gammab_{c}}

\newcommand{\psib}{\boldsymbol{\psi}}


%%MODEL
\newcommand{\hyper}{g_{\phi}}
\newcommand{\inr}{f_{\theta}}

%%%%%%%%%% OPERATIONS

\newcommand{\Eme}[2][]{
  \bgroup
  \ifx\relax#1\relax
    \E\left[ #2 \right]
  \else
    \E_{#1}\left[ #2 \right]
  \fi
  \egroup
}

%%%
% KL-divergence
%
%   \kld{p}{q}
%%%

% \DeclarePairedDelimiterX{\infdivx}[2]{(}{)}{%
  % #1||#2%
% }
\newcommand{\klme}[2]{\ensuremath{\KL\left(#1 \Vert #2\right)}}

\newcommand{\normald}{\mathcal{N}}
% \newcommand{\nop}{\ignorespaces}
% \newcommand{\pages}[1]{\nop}


==> tikz.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% LIBRARIES
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\RequirePackage{tikz,pgfplots}

\usetikzlibrary{
    shapes,
    pgfplots.groupplots,
    shadings,
    calc,
    arrows,
    backgrounds,
    colorbrewer,
    shadows.blur,
    external,
    shapes,
    shapes.arrows,
    shapes.symbols,
    arrows.meta,
    positioning, 
    decorations.pathreplacing,
    intersections,
    cd,
    babel, % otherwise there is an error when importing spanish in babel
    fit % For extending the bounding box
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% STYLES
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\tikzstyle{varcurvestyle}=[
    smooth,
    thick,
    mark=none,
    domain=1:1000,
    samples=100,
]

\tikzstyle{ballstyle}=[
    smooth,
    thick,
    mark=none,
%    domain=-1:1,
    samples=500,
]
